Linking Social Media Posts to News with Siamese Transformers

Many computational social science projects examine online discourse surrounding a specific trending topic. These works often involve the acquisition of large-scale corpora relevant to the event in question to analyze aspects of the response to the event. Keyword searches present a precision-recall trade-off and crowd-sourced annotations, while effective, are costly. This work aims to enable automatic and accurate ad-hoc retrieval of comments discussing a trending topic from a large corpus, using only a handful of seed news articles.

==> figures/images/density_plots.tex <==
For each model, we present the precision and the number of true positives. Each column is the threshold of cosine similarity at which a positive classification was made. Interestingly, S-ASTRA shows worse precision at lower thresholds, but returns far more true positives at higher confidence thresholds with reasonable to strong precision. Figure \ref{fig:kde} visually explains this outcome using the cosine similarity densities between article and comment pairs learned by both S-ASTRA and a GRU. Cosine similarities of positive (relevant) pairs are shown in green, and irrelevant (negative) pairs in red. The GRU is generally less certain in its estimations, while S-ASTRA is able to learn more confident relations between pairs, resulting in greater densities at higher levels of certainty.


\begin{figure}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{figures/StarTransformer.pdf}
  \caption{Star Transformer}
  \label{fig:sub1}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{figures/gru.pdf}
  \caption{GRU.}
  \label{fig:sub2}
\end{subfigure}
\caption{Density plots of article-tweet cosine similarities.}
\label{fig:kde}
\end{figure}

==> figures/tables/old.tex <==
\begin{table}[htpb]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
 & \multicolumn{1}{c|}{\textbf{0.7}} & \multicolumn{1}{c|}{\textbf{0.85}} & \multicolumn{1}{c|}{\textbf{0.9}} & \multicolumn{1}{c|}{\textbf{0.95}} & \multicolumn{1}{c|}{\textbf{0.975}} & \multicolumn{1}{c|}{\textbf{0.99}} \\ \hline
\textbf{CNN} & 0.22 (2352) & 0.86 (850) & 0.97 (259) & 1.0 (7) & N/A & N/A \\ \hline
\textbf{GRU} & 0.15 (2229) & 0.69 (819) & 0.86 (216) & 1.0 (9) & N/A & N/A \\ \hline
\textbf{Bi-GRU} & 0.33 (1888) & 0.84 (390) & 0.90 (71) & N/A & N/A & N/A \\ \hline
\textbf{S-ASTRA} & 0.04 (2775) & 0.27 (2176) & 0.45 (1750) & 0.64 (907) & 0.75 (348) & 0.87 (76) \\ \hline
\textbf{S-ASTRA$^2$} & 0.15 (2212) & 0.42 (573) & 0.64 (216) & 0.99 (84) & 1.0 (46) & N/A \\ \hline
\end{tabular}
\caption{Precision and true positives on the test set (3307 samples).}
\label{tab:twitter}
\end{table}
